Beyond Leaderboards: A survey of methods for revealing weaknesses in Natural Language Inference data and models

Recent years have seen a growing number of publications that analyse Natural Language Inference (NLI) datasets for superficial cues, whether they undermine the complexity of the tasks underlying those datasets and how they impact those models that are optimised and evaluated on this data. This structured survey provides an overview of the evolving research area by categorising reported weaknesses in models and datasets and the methods proposed to reveal and alleviate those weaknesses for the English language. We summarise and discuss the findings and conclude with a set of recommendations for possible future research directions. We hope it will be a useful resource for researchers who propose new datasets, to have a set of tools to assess the suitability and quality of their data to evaluate various phenomena of interest, as well as those who develop novel architectures, to further understand the implications of their improvements with respect to their model's acquired capabilities.

==> figures/by_dataset.tex <==
\begin{tikzpicture}
\begin{axis}[
height=13em,
    width  = \textwidth,
    ybar=0.5pt,
    ymin=0,
    ymax=100,
    scaled y ticks = false,
    bar width=2pt,
    x tick label style={rotate=30, anchor=east, align=right,text width=2cm, font=\scriptsize\itshape},
    major x tick style = transparent,
    ylabel={\# papers},
    xmajorgrids=true,
    x tick label as interval,
    ymajorgrids=true,
    y grid style=dashed,
    legend columns=-1,
    %xticklabels={Redundancy,Lex Entailment,Dative,Synonym,Abbreviation,Symmetry,Nomi\-nalisation,Genitive,Voice,Restrictivity,Factivity,Coreference,Ellipsis/Implicit,Preposition,Listing,Scope,RelAdvApp},
    xtick={0,1,2,3,4,5,6,7},
    xmin=0, xmax=8,
        ]
%     \addplot+[legend entry=\textsc{MSMarco}, color=bblue, fill=bblue] 
% coordinates {
%     (0.5,40) (1.5,0) (2.5,0) (3.5,23) (4.5,7) (5.5,0) (6.5,0) (7.5,0) (8.5,7) (9.5,0) (10.5,0) (11.5,23) (12.5,7) (13.5,0) (14.5,0) (15.5,0) (16.5,0)
%     };
% \addplot+[legend entry=\textsc{HotpotQA}, color=rred, fill=rred] 
% coordinates {
%     (0.5,76) (1.5,2) (2.5,0) (3.5,14) (4.5,8) (5.5,0) (6.5,12) (7.5,0) (8.5,8) (9.5,0) (10.5,0) (11.5,64) (12.5,6) (13.5,2) (14.5,32) (15.5,0) (16.5,40)
%     };
% \addplot+[legend entry=\textsc{ReCoRd}, color=ggreen, fill=ggreen] 
% coordinates {
%     (0.5,44) (1.5,2) (2.5,0) (3.5,58) (4.5,2) (5.5,0) (6.5,0) (7.5,0) (8.5,5) (9.5,0) (10.5,0) (11.5,60) (12.5,7) (13.5,0) (14.5,12) (15.5,0) (16.5,7)
%     };
% \addplot+[legend entry=\textsc{MultiRC}, color=ppurple, fill=ppurple] 
% coordinates {
%     (0.5,63) (1.5,4) (2.5,0) (3.5,22) (4.5,2) (5.5,0) (6.5,2) (7.5,0) (8.5,2) (9.5,0) (10.5,2) (11.5,69) (12.5,6) (13.5,0) (14.5,12) (15.5,0) (16.5,8)
%     };
% \addplot+[legend entry=\textsc{NewsQA}, color=pink, fill=pink] 
% coordinates {
%     (0.5,71) (1.5,0) (2.5,0) (3.5,39) (4.5,0) (5.5,0) (6.5,0) (7.5,0) (8.5,3) (9.5,0) (10.5,0) (11.5,29) (12.5,3) (13.5,0) (14.5,3) (15.5,0) (16.5,21)
%     };
% \addplot+[legend entry=\textsc{DROP}, color=teal, fill=teal] 
% coordinates {
%     (0.5,60) (1.5,0) (2.5,0) (3.5,24) (4.5,14) (5.5,0) (6.5,4) (7.5,0) (8.5,4) (9.5,0) (10.5,0) (11.5,14) (12.5,16) (13.5,0) (14.5,26) (15.5,0) (16.5,6)
%     };
% \begin{pgfonlayer}{background}
%   \fill[color=black!10] (axis cs:0,0) rectangle (axis cs:6,100);
% \end{pgfonlayer}
% \begin{pgfonlayer}{background}
%   \fill[color=black!10] (axis cs:9,0) rectangle (axis cs:13,100);
% \end{pgfonlayer}
\end{axis}
\end{tikzpicture}

==> figures/by_task.tex <==
\def\angle{20}
\def\radius{2.5}
\def\cyclelist{{"bblue","rred", "pink", "ggreen"}}
\newcount\cyclecount \cyclecount=-1
\newcount\ind \ind=-1
\begin{tikzpicture}[nodes = {font=\sffamily}]
\foreach \percent/\name in {
50.72 / RTE(35),
36.23 / MRC(25),
7.25 / Multiple(5),
5.80 / Other(4)
} {
      \ifx\percent\empty\else               % If \percent is empty, do nothing
        \global\advance\cyclecount by 1     % Advance cyclecount
        \global\advance\ind by 1            % Advance list index
        \ifnum3<\cyclecount                 % If cyclecount is larger than list
          \global\cyclecount=0              %   reset cyclecount and
          \global\ind=0                     %   reset list index
        \fi
        \pgfmathparse{\cyclelist[\the\ind]} % Get color from cycle list
        \edef\color{\pgfmathresult}         %   and store as \color
        % Draw angle and set labels
        \draw[fill={\color!50},draw={\color}] (0,0) -- (\angle:\radius)
          arc (\angle:\angle+\percent*3.6:\radius) -- cycle;
        \node at (\angle+0.5*\percent*3.6:0.7*\radius) {\percent\,\%};
        \node[pin=\angle+0.3*\percent*3.6:\name]
          at (\angle+0.3*\percent*3.6:\radius) {};
        \pgfmathparse{\angle+\percent*3.6}  % Advance angle
        \xdef\angle{\pgfmathresult}         %   and store in \angle
      \fi
    };
\end{tikzpicture}

